Assessing Treatment Effect Variation in Observational Studies: Results from a Data Challenge

A growing number of methods aim to assess the challenging question of treatment effect variation in observational studies. This special section of "Observational Studies" reports the results of a workshop conducted at the 2018 Atlantic Causal Inference Conference designed to understand the similarities and differences across these methods. We invited eight groups of researchers to analyze a synthetic observational data set that was generated using a recent large-scale randomized trial in education. Overall, participants employed a diverse set of methods, ranging from matching and flexible outcome modeling to semiparametric estimation and ensemble approaches. While there was broad consensus on the topline estimate, there were also large differences in estimated treatment effect moderation. This highlights the fact that estimating varying treatment effects in observational studies is often more challenging than estimating the average treatment effect alone. We suggest several directions for future work arising from this workshop.

==> input/introduction.tex <==

\section{Introduction}
\label{sec:introduction}

Workshop conducted at the 2018 Atlantic Causal Inference Conference at
Carnegie Mellon University in Pittsburgh, Pennsylvania.

\subsection{Data description}
\label{sec:description}

The analyzed dataset was based on preliminary data extracted from the
National Study of Learning Mindsets
\footnote{\url{http://mindsetscholarsnetwork.org/about-the-network/current-initatives/national-mindset-study/}}. This
is a study that evaluates a ``nudge-like'' intervention to change
student behavior at very low cost, but seeks to understand
heterogeneity in the intervention. The main goal of the study is to
test for heterogeneity in the effect of an intervention designed to
instill students with a ``growth mindset''
\footnote{\url{http://mindsetscholarsnetwork.org/learning-mindsets/growth-mindset/}}.
A growth mindset is the belief that intelligence can be developed. It
is contrasted with a fixed mindset, the belief that intelligence is an
innate trait that is fixed from birth. Because growth mindset
interventions only teach students to see their school differently, but
don't try to change schools themselves, then growth mindset
interventions are thought to depend in important ways on the school
context. But research has not yet interrogated treatment effect
heterogeneity sufficiently.

The National Study of Learning Mindsets was a randomized controlled
trial in a national probability sample of U.S. public high
schools. For the purpose of this workshop we created a dataset that
instead emulates an observational study with similar characteristics
as the National Study (including covariate distributions, data
structures, and effect sizes).  Attached is a dataset of about 10,000
students in 76 schools with a simulated outcome $Y$ (a continuous
measure of achievement), a binary treatment variable $Z$ indicating
receipt of the intervention, and the following ten covariates, the
first four of which are measure at the student level and remaining six
measured at the school level (Table~\ref{tab:data-description}).

\begin{singlespacing}
    \begin{table}[ht]
      \centering
      \begin{tabular}[ht]{ | l | p{0.5\textwidth} | } \hline Covariate
           & Description                                                                                                                        \\ \hline
        S3 & Student's self-reported expectations for success in the future, a proxy for prior achievement, measured prior to random assignment \\ \hline
        C1 & Categorical variable for student race/ethnicity                                                                                    \\ \hline
        C2 & Categorical variable for student identified gender                                                                                 \\ \hline
        C3 & Categorical variable for student first-generation status (i.e., first in family to go to college)                                  \\ \hline \hline
      % -------------------------------------------------------------------------
        XC & School-level categorical variable for urbanicity of the
                      school (i.e., rural, suburban, etc.)                                                                                      \\ \hline
        X1 & School-level mean of students' fixed mindsets, reported
                         prior to random assignment                                                                                             \\ \hline
        X2 & School achievement level, as measured by test scores and
                         college preparation for the previous four cohorts of students                                                          \\ \hline
        X3 & School racial/ethnic minority composition -- i.e.,
                         percentage black, Latino, or Native American                                                                           \\ \hline
        X4 & School poverty concentration -- i.e., percentage of
                         students who are from families whose incomes fall below the federal
                         poverty line                                                                                                           \\ \hline
        X5 & School size -- Total number of students in all four grade
                         levels in the school                                                                                                   \\ \hline
      \end{tabular}
      \caption{Covariate description}
      \label{tab:data-description}
    \end{table}

\end{singlespacing}

% % Itemized list of covariates
% \begin{singlespacing}
%     \begin{itemize}
%   \item S3 -- Student's self-reported expectations for success in the
% future, a proxy for prior achievement, measured prior to random
% assignment
%   \item C1 -- Categorical variable for student race/ethnicity
%   \item C2 -- Categorical variable for student identified gender
%   \item C3 -- Categorical variable for student first-generation status
%     (i.e., first in family to go to college)
%   \item XC -- School-level categorical variable for urbanicity of the
%     school (i.e., rural, suburban, etc.)
%   \item X1 -- School-level mean of students' fixed mindsets, reported
%     prior to random assignment
%   \item X2 -- School achievement level, as measured by test scores and
%     college preparation for the previous four cohorts of students
%   \item X3 -- School racial/ethnic minority composition -- i.e.,
%     percentage black, Latino, or Native American
%   \item X4 -- School poverty concentration -- i.e., percentage of
%     students who are from families whose incomes fall below the federal
%     poverty line
%   \item X5 -- School size - Total number of students in all four grade
%     levels in the school
%   \end{itemize} 
% \end{singlespacing}


\subsection{Research questions}
\label{sec:research-questions}

\begin{enumerate}
\item Was the mindset intervention effective in improving student
achievement?
\item Researchers hypothesize that the effect of the intervention is
moderated by school level achievement (X2) and pre-existing mindset
norms (X1). In particular there are two competing hypotheses about
how X2 moderates the effect of the intervention: Either it is
largest in middle-achieving schools (a ``Goldilocks effect'') or is
decreasing in school-level achievement
\item Researchers also collected other covariates and are interested in
exploring their possible role in moderating treatment effects.
\end{enumerate}

\subsection{Participants}
\label{sec:participants}

In total there were nine participants in the workshop, who all gave
presentations of their findings.  Here we list the presenters by order
of appearance, along with a brief description of their choice of methodology:

\begin{singlespacing}
  \begin{itemize}
  \item Stefan Wager (Stanford): Random forests using the R-Learner
    objective (Robinson transformation)
  \item Alejandro Schuler (Stanford): Shallow CART fit to Robinson-transformed
    outcome from R-Learner.
  \item Luke Keele (Penn) and Sam Pimentel (UC-Berkeley): Matching.
  \item Qingyuan Zhao (Penn): Linear model on a transformed outcome
    and treatment with lasso regularization, and selection adjustment
    for nonzero coefficients.  
  \item \Soeren \Kuenzel (UC-Berkeley): Use multiple HTE detection
    methods to detect candidate subgroups, and use standard ATE
    estimators within these subgroups.
  \item Nicole Carnegie (Montana State) and Jennifer Hill (New York
    University): Bayesian additive regression trees (BART)
  \item Alexander Volfovsky (Duke): Matching after learning to stretch
    (MALTS), a new variant of the matching framework.
  \item Frederik Johannsson (MIT): Ridge regression, neural networks,
    and random forests.  
  \item Bryan Keller (Columbia): Propensity score matching.
  \end{itemize}  
\end{singlespacing}

All presenters, with the exception of Schuler, submitted a written
report, usually accompanied by one or more coauthors.  These
submissions are all included in this issue.  

% Written submissions were given by, in alphabetical order by first
% author.

% \begin{singlespacing}
%   \begin{itemize}
%   \item Susan Athey (Stanford) and Stefan Wager (Stanford)
%   \item Nicole Carnegie (Montana State), Vincent Dorie (Columbia), and
%     Jennifer Hill (New York University)
%   \item Frederik Johannsson (MIT)
%   \item Luke Keele (Penn) and Sam Pimentel (UC-Berkeley)
%   \item Bryan Keller (Columbia), Jiashen Chen (Education Testing
%     Services), and Tianyang Zhang (Columbia)
%   \item \Soeren \Kuenzel (UC-Berkeley), Simon J.S. Walter (UC-Berkeley), and Jasjeet
%     S. Sekhon (UC-Berkeley)
%   \item Harsh Parikh (Duke), Alexander Volfovsky (Duke), and Cynthia
%     Rudin (Duke)
%   \item Qingyuan Zhao (Penn) and Snigdha Panigrahi (Michigan)
%   \end{itemize}
% \end{singlespacing}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> input/summary-findings.tex <==

\section{Summary of findings}
\label{sec:summary-findings}

% Here we briefly summarize the authors' respective responses to the
% research questions.

There was consensus in interpretation by the authors that Question 1
concerns estimation of the average treatment effect (ATE).
Tables~\ref{tab:ATE-summary} shows estimates and uncertainty bounds
for the ATE.  There is striking agreement between authors for both
quantities, showing strong support for a large \textcolor{blue}{(is it
  justified to call it large? i.e. signal-to-noise ratio)} positive,
despite the divergence in the nature of their respective modeling
choices.  This fact is quite noteworthy; some authors calculated the
ATE by using nonparametric regression to impute individual treatment
effects (ITEs) and taking the empirical average of the ITEs, and some
used simple propensity-weighted estimators, but these two approaches
and everything in between all returned very similar ATE estimates.
Though this finding could be particular to this synthetic dataset, it
raises the possibility of the robustness of ATE estimation to modeling
choices, at least for large sample sizes.

Responses to Question 2, regarding effect modification by the
pre-specified covariates X1 and X2, are show in
Table~\ref{tab:question-2}.  In contrast to the ATE estimates, there
is considerable disagreement among conclusions of effect modification.
On the one hand, there is general agreement around X1 having a
mitigating effect on treatment efficacy. On the other hand, the
findings range widely in their strength of support of modification
mediated by X2, though all those who support the existence of effect
modification determined there to be an increasing trend.

Similarly, there are mixed levels of overlap in the responses to
Question 3, shown in Table~\ref{tab:question-3}, regarding the
existence of effect modification by other covariates.  Nearly every
author, with the exception of Athey \& Wager, determined XC to
negatively impact the treatment effect.  However, two authors reported
S3 to have an increasing trend in treatment effect, while all other
authors did not report this finding.

It should be noted that most investigations into effect modification
are \textit{ad hoc} in their nature, and widely differed in their
standard of evidence.  For instance, some conclusions were based
purely on qualitative inspections of partial dependence plots.  Others
were based on dividing individuals by their quantile in the suspected
effect modifier, and estimating the ATE within these subgroups.
However, there is no obvious principled way to choose the granularity
of these candidate subgroups.  In fact, the level of granularity was
often chosen after inspecting partial dependence plots, so typical
significance tests for difference in means will no longer have the
usual frequentist properties.

\begin{table}[ht]
  \centering
  \begin{tabular}[ht]{|l|r|}
    \hline
    Author            & ATE estimate (95 \% C.I.)$^{\dagger}$ \\ \hline
    Athey \& Wager    & 0.25 (0.21, 0.29)                     \\ 
    Carnegie et al.   & 0.25 (0.23, 0.27)                     \\ 
    Johannsson        & 0.27 (0.22, 0.31)                     \\ 
    Keele \& Pimentel & 0.27 (0.25, 0.30)                     \\
    Keller et al.     & 0.26 (0.22, 0.30)                     \\ 
    \Kuenzel et al.   & 0.25 (0.22, 0.27)                     \\ 
    Parikh et al.     & 0.26 (0.25, 0.26)                     \\ 
    Zhao \& Panigrahi & 0.26 (0.24, 0.28)                     \\ \hline
  \end{tabular}
  \caption{Answers to Question 1 concerning the average treatment
    effect (ATE). $^\dagger$All intervals are confidence intervals,
    except for Carnegie et al., who provide credible intervals. }
  \label{tab:ATE-summary}
\end{table}

\begin{table}[ht]
  \centering
  \begin{tabular}{|l|p{5cm}|p{5cm}|}
    \hline
    Author            & X1                 & X2                    \\ \hline
    %
    %
    Athey \& Wager    & \textbf{Moderate support} for decreasing trend
                        in treatment effect, though  mitigated after controlling for other variables.    & \textbf{No.}  \\ \hline
    %
    %
    Carnegie et al.   & \textbf{Yes}, decreasing trend in treatment effect. & \textbf{Yes}, an increasing trend in, though without evidence of a Goldilocks effect \\ \hline
    %
    %
    Johannsson        & \textbf{Yes}, decreasing trend in treatment effect. &     \textbf{No.}  \\ \hline
    %
    %
    Keele \& Pimentel & \textbf{Yes}, decreasing trend in treatment effect, though confidence intervals for quintiles overlap.  & \textbf{Moderate support}; lowest quintile has lower treatment effect, though little separation among other quintiles.  \\ \hline
    %
    %
    Keller et al.     & \textbf{Moderate support} from exploratory analysis.    &  \textbf{Moderate support} for presence Goldilocks effect. \\ \hline
    %
    %
    \Kuenzel et al.   & \textbf{Yes}. increasing trend in treatment effect.   & \textbf{No}, though there is cursory evidence in CATE plots. \\ \hline
    %
    %
    Parikh et al.     & \textbf{Yes}, increasing then decreasing trend in treatment effect.   &  \textbf{Yes}, exploratory support for Goldilocks effect.   \\ \hline
    %
    %
    Zhao \& Panigrahi & \textbf{Yes}, though negative effect modification is insignificant after selection adjustment.   & \textbf{No.} \\ 
    \hline
  \end{tabular}
  \caption{Answers to Question 2 concerning effect modification by X1
    and X2}
  \label{tab:question-2}
\end{table}

\begin{table}[ht]
  \centering
  \begin{tabular}{|l|p{7cm}|}
    \hline
    Author & Other effect modifiers found \\ \hline
    Athey \& Wager    & \textbf{None.} \\ \hline
    Carnegie et al.   & \textbf{XC} = 3 has much lower treatment
                        effect; Top two levels of \textbf{S3} have
                        higher treatment effects compared to other levels. \\ \hline
    Johannson         & \textbf{XC} = 3 has a lower treatment effect; \textbf{S3} has an increasing trend in treatment effect. \\ \hline
    Keele \& Pimentel & \textbf{XC} is an effect modifier, though there is only exploratory evidence for this. \\ \hline
    Keller et al.     & \textbf{XC} = 3 has a lower treatment effect, but this finding is not robust to propensity score modeling choice.\\ \hline
    Parikh et al.     & \textbf{XC} = 3 has a lower treatment effect. \\ \hline
    \Kuenzel et al.         & \textbf{XC} = 3 has a lower treatment effect. \\ \hline
    Zhao \& Panigrahi & \textbf{XC} = 3 has a lower treatment effect. \\ \hline
  \end{tabular}
  \caption{Answers to Question 3 concerning other possible effect
    modifiers besides X1 and X2}
  \label{tab:question-3}
\end{table}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> input/synthesis.tex <==

\section{Synthesis}
\label{sec:common-themes}

In synthesizing the contributed papers, we focus on three main areas.
First,

\paragraph{Making substantive questions statistically precise}

As with all real-world analyses, there are important open-ended
questions in terms of translating the substantive goals of the
research study with corresponding statistical methods.  Deciding the
ultimate goal of the exercise can be paramount for choosing between
approaches.  One aspect of defining this goal may be framed as a
choice between two alternatives.  Are researchers fundamentally
interested in foundational scientific questions and the ``mechanism''
by which the intervention works?  Are they instead focused on making
specific policy decisions, such as whether to roll out the
intervention at scale or to a specific subgroup?  Framing this tension
in statistical terms: which questions and hypotheses are exploratory
and which are confirmatory, and when does such a distinction matter?

The considered methods widely differ in their approach.  On one
extreme, Zhao and Panigrahi have different inferential procedures for
pre-determined candidate subgroup effects (school-level fixed mindset
X1 and achievement level X2, as specified in Question 2) versus
``discovered'' subgroup effects, as mentioned in Question 3.  They use
the arguments of \cite{berk2013} and \cite{Fithian} that using the
same data for both discovery and estimation of effect modification
will generally result in selection bias.  This motivates their
approach of using the likelihood conditional on and truncated to the
selection event from the lasso \citep{lee2016}.  Of course, one
downside is that tools for selective inference have so far only been
developed for variable selection in the linear model. misspelled. 

At the other extreme, Carnegie et al. treat all variation the same,
and conduct their investigation into treatment effect heterogeneity by
leveraging posterior uncertainty from BART. Most approaches lie
between these two extremes, including sample splitting (\Kuenzel et
al.), and masking the sign of the impact (Keele and
Pimentel). However, these methods can reduce statistical power to
detect effect modification by reducing the amount of data used for
estimation. Keller et al. select the penalization parameter for their
CART fit to treatment effects by controlling type-I error as
calculated by a permutation scheme. 


\paragraph{Separating flexible modeling from final questions}

Remarkably, nearly every submission took a similar approach to detect
and describe treatment effect modification.  First, fit a flexible
model, including BART (Carnegie et al.), matching (Keller et al.;
Parikh et al.), random forest (Athey \& Wager), neural network
(Johannson), etc., to impute individual treatment effects for each
student.  Second, report a low-dimensional summary to the fit from the
first stage.  Approaches to this second step included smoothing
school- or student-level ITE estimates as a function of the covariate
of interest (producing something similar to a partial dependence
plot), fitting a CART to the estimated ITEs, and even simply a linear
model.  These are all familiar tools to most researchers, and lend
themselves well to easy interpretation and graphical representation.  

This is clearly an attractive approach, as it allows for some degree
of internal consistency and coherency across subgroup estimates.  For
instance, the same ``flexible'' individual-level estimates are
aggregated in different ways to look at variation across both school
achievement and pre-existing mindset norms.  Another advantage is
interpretability, as the presented models are typically
difficult to describe as a consequence of their flexible nature. 

Still, this two-step approach raises several open-ended statistical
questions.  While generally valid from a Bayesian perspective, as it
simply entails characterization of the posterior distribution after
conditioning on the data only once \citep*{BCF}, the frequentist
properties of such a procedure are still unclear, as pointed out by
Zhao \& Panigrahi.  Applying a strict selective inference framework
such as theirs to this setting seems untenable, as it is difficult to
characterize the stochastic process by which effect modifiers are
detected in this way.  More broadly, is repeatedly using the
first-stage estimates asking too much of the first-stage model?
Certainly the estimation trade-offs (e.g., level of regularization)
might be different for 

Even from an exploratory framework, a subtle yet important issue is
that, analogous to Simpson's paradox, the sign of the estimated
treatment effect can vary depending on the level of aggregation
(\textcolor{blue}{Avi wanted to cite ``Tyler VdW'' here [Tyler
  VanderWeele?] here}).  Thus, even with data from a randomized trial,
there is no ``correct'' level of aggregation.  This introduces
additional trade-offs, as well as researcher degrees of freedom.
Guiding principles for this two-stage approach, such as when to
account for interactive effects, have yet to be established. 

\paragraph{Tailoring methods for an observational studies}

The (simulated) data for this data challenge come from an
observational study rather than a randomized trial. Therefore, a
appropriately accounting for confounding is a first-order practical
concern here.  This is particularly challenging when researchers are
interested in treatment effect variation; when a method only partially
accounts for confounding, it is easy to confuse differential
confounding for varying treatment effects.

It is common to check for global covariate balance when estimating
overall impact in an observational study. A natural extension to
heterogeneous treatment effect estimation would be to also check for
\emph{local} covariate balance, such as separately by candidate
subgroups.  Such analyses were largely absent from the contributed
papers, suggesting that the field should develop standards in this
area. 

Another element that is critical for observational studies is
assessing to violations of the unconfoundedness assumption.  Keele \&
Pimentel assess sensitivity within the matching framework; Carnegie et
al. instead use a model-based approach, and \Kuenzel et al. use a
permutation approach.  While important, such analyses are inherently
difficult and limited, since existing approaches to sensitivity
largely assume that the impact of the unmeasured confounder is
constant across the covariate space -- or adapt a minimax approach.
Some recent papers have began to push in this direction.
(\textcolor{blue}{Avi wanted to cite something here too. Though it
  seems to me that, unless you make some assumption on what ``shape''
  the unmeasured confounding has across the covariate space, it is
  difficult to distinguish the treatment effect from the unmeasured
  confounding [reminds me of the spatial confounding / UQ literature]
}).


There is a marked difference in level of emphasis put on the
observational aspect of the data exercise, with some methods more
(\textcolor{blue}{Examples / explanations?}). Approaches included
applying the Robinson transformation \citep{Robinson, RLearner} to the
treatment and outcome variables (Athey \& Wager, Zhao \& Panigrahi),
conditioning on the propensity score (Carnegie et al.; Keller et al.),
and matching to emulate a randomized control trial (Keele \& Pimentel,
and to a lesser extent Parikh et al.).  Understanding when tools from
randomized trials can be used without modification, or with only
modest modification, is an important area for future work.

\textcolor{blue}{Parikh et al. suggest that their strange matching approach lends
itself to ``locate possible sources of confounding\ldots'' is this
true\ldots? And is it OK to use the outcome to determine matches? }



\paragraph{Other points}

\subparagraph{Modeling the multilevel structure of data}

The main motivation of this workshop was to detect treatment effect
heterogeneity, and possibly as a result of this, modeling the
multilevel structure of the data became a secondary
objective. Approaches included using ``cluster-robust'' random forests
(Wager \& Athey), bootstrapping and sampling splitting at the school
level (Johannson; \Kuenzel et al.), including fixed or random effects
at the school level (Carnegie et al.), and considering matching both
between and within schools (Keele \& Pimentel). 

\subparagraph{Consistency of ATE estimates from different approaches}

As demonstrated in Table~\ref{tab:ATE-summary}, despite the diversity
of statistical methods employed, most analyses resulted in remarkably
similar estimates and uncertainty bounds for the average treatment
effect.  Conversely, Tables~\ref{tab:question-2} and
\ref{tab:question-3} and show that current methods to detect treatment
heterogeneity often do not agree. It is worth noting that rarely do
presented results directly contradict one another. While some methods
reported discovered effect modifiers that others failed to detect, no
two methods, for example, found effect modification trends happening
in opposite directions.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

